LiResolver: License Incompatibility Resolution for Open Source Software

Open source software (OSS) licenses regulate the conditions under which OSS can be legally reused, distributed, and modified. However, a common issue arises when incorporating third-party OSS accompanied with licenses, i.e., license incompatibility, which occurs when multiple licenses exist in one project and there are conflicts between them. Despite being problematic, fixing license incompatibility issues requires substantial efforts due to the lack of license understanding and complex package dependency. In this paper, we propose LiResolver, a fine-grained, scalable, and flexible tool to resolve license incompatibility issues for open source software. Specifically, it first understands the semantics of licenses through fine-grained entity extraction and relation extraction. Then, it detects and resolves license incompatibility issues by recommending official licenses in priority. When no official licenses can satisfy the constraints, it generates a custom license as an alternative solution. Comprehensive experiments demonstrate the effectiveness of LiResolver, with 4.09% false positive (FP) rate and 0.02% false negative (FN) rate for incompatibility issue localization, and 62.61% of 230 real-world incompatible projects resolved by LiResolver. We discuss the feedback from OSS developers and the lessons learned from this work. All the datasets and the replication package of LiResolver have been made publicly available to facilitate follow-up research.

==> background.tex <==
\section{Background}\label{sec:background}
\subsection{OSS License}
Among them, license information of all OSS presences, may appear in independent license files (e.g., LICENSE, COPYING) called \textit{Declared License}, in the comment texts in the top header of code files called \textit{Inline License}, or in license names only or license implied by third-party packages called \textit{Referenced License}.  

%As previous studies~\cite{xu2021lidetector}, t
The declared and inline licenses can be directly obtained from the license file (e.g., LICENSE.txt) and at the beginning of source code files, respectively. The referenced licenses are obtained according to the referenced license name, version or imported third-party software packages whose licenses can be found from external sources like the Python Package Index~\cite{url-pypi}, SPDX~\cite{mancinelli2006managing,url-spdx-licenses}, and the hosted pages for OSS licenses.


The terms of licenses...

Three types of licenses...

\noindent \textbf{Official licenses \textit{vs.} license exceptions \textit{vs.} custom licenses}

%\noindent \textbf{Project license}

%\noindent \textit{Component license}


\subsection{License Incompatibility}
MPL and GPL.
MIT
%\noindent \textbf{Incompatibility between project and component licenses}

%\noindent \textbf{Component licenses \textit{vs.} component license}

\subsection{Motivating Study}
